Networked Restless Bandits with Positive Externalities

Restless multi-armed bandits are often used to model budget-constrained resource allocation tasks where receipt of the resource is associated with an increased probability of a favorable state transition. Prior work assumes that individual arms only benefit if they receive the resource directly. However, many allocation tasks occur within communities and can be characterized by positive externalities that allow arms to derive partial benefit when their neighbor(s) receive the resource. We thus introduce networked restless bandits, a novel multi-armed bandit setting in which arms are both restless and embedded within a directed graph. We then present Greta, a graph-aware, Whittle index-based heuristic algorithm that can be used to efficiently construct a constrained reward-maximizing action vector at each timestep. Our empirical results demonstrate that Greta outperforms comparison policies across a range of hyperparameter values and graph topologies.

==> proofs/w1_leq_wq2.tex <==
\begin{restatable}[]{lemma}{w1leqw2}\label{thm:w1leqw2}
Given a set of active actions $\mathcal{A}^\prime := \{a | a \in \mathcal{A} \setminus 0 \}$, and any restless or collapsing arm $i \in [n]$ whose transition matrices satisfy the structural constraints outlined in Section~\ref{sec:model}, for any ordered pair of active actions $(a,a^\prime) \in \mathcal{A}^\prime  \times \mathcal{A}^\prime $, and belief state at time $t$, $b_t^i \in [0,1]$, $a < a^\prime \rightarrow W_a(b_t^i) < W_{a^\prime}(b_t^i)$. 
\end{restatable}

\begin{proof}
Recall from Section~\ref{sec:algDetails} that for active action $\alpha \in \mathcal{A}^\prime $ and arm $i$ with belief state $b_t^i \in [0,1]$, the Whittle index represents the infimum subsidy, $m$, required to make arm $i$ indifferent between passivity (i.e., receipt of a \texttt{no-act}) and receipt of active action $\alpha$. Formally:
\begin{equation}
\label{eq:whittle}
 W_\alpha(b_t^i) = \inf_m \{m \mid V_m(b_t^i, a_t^i = 0) \geq V_m(b_t^i, a_t^i = \alpha)\}
\end{equation}
where $V_m$ represents the value function as defined in Equation~\ref{eqn:valueFunc} and repeated for convenience below:
\begin{equation}
\begin{aligned}
    \label{eqn:valueFuncApp}
    V_m(b_t^i) = 
    \max \begin{cases}
    m + r(b_t^i) + \beta V_m \left(b_{t+1}^i\right) & \textit{no-act} \\
    r(b_t^i)+\beta [b_t^i V_m\left(P^{\alpha}_{1,1}\right) + 
    (1-b_t^i) V_m\left(P^{\alpha}_{0,1}\right)]  
    & \textit{$\alpha$}
    \end{cases}
    \end{aligned}
\end{equation}

Recall from Section~\ref{sec:model} that structural constraint (ii) states:
$$\forall (a, a^\prime) \in \mathcal{A} \times \mathcal{A}, a < a^\prime \rightarrow P^a_{0,1} < P^{a^\prime}_{0,1}; P^a_{1,1} < P^{a^\prime}_{1,1}$$

Thus, $a < a^\prime \rightarrow$:
\begin{equation}
b_t^i V_m\left(P^{a}_{1,1}\right) + (1-b_t^i) V_m\left(P^{a}_{0,1}\right) < b_t^i V_m\left(P^{a^\prime}_{1,1}\right) + (1-b_t^i) V_m\left(P^{a^\prime}_{0,1}\right)
\end{equation}

From here, it follows that for any given subsidy, $m$, for which the active term of the value function is the max term,
$$V_m(b_t^i,  a_t^i = 0) < V_m(b_t^i,  a_t^i = a) < V_m(b_t^i, a_t^i = a^\prime)$$

Thus, $$\inf_m \{m \mid V_m(b_t^i, a_t^i = 0) \geq V_m(b_t^i, a_t^i = a)\} < \inf_m \{m \mid V_m(b_t^i, a_t^i = 0) \geq V_m(b_t^i, a_t^i = a^\prime)\}$$
\end{proof}
